Not All Who Wander Are Lost: Early Excess Demographics in the Volume-limited ZTF DR2 SN Ia Sample

Early-time flux excesses in Type Ia supernovae (SNe~Ia) offer a unique insight into their progenitor systems and explosion mechanisms. Although individual early-excess events and larger searches have been reported, demographic studies remain limited by sample size. We present a systematic search for early-time excess emission in a volume-limited sample ($z<0.06$) of SNe~Ia based on the Zwicky Transient Facility Data Release 2 (ZTF DR2). Using ZTF $g$- and $r$-band light curves, we identify candidates showing early-excesses shortly after the explosion time, and we apply conservative coverage and quality requirements to build reliable ``excess'' and ``no-excess'' bump and no-bump catalogs. From an initial sample of 1547 SNe~Ia, our final catalogs contain 42 early-excess and 110 no-excess events. We compare the two populations using SN and host environment parameters from ZTF DR2 and quantify the differences using two-sample statistical tests. We find the strongest differences are in SN light-curve properties: early-excess events have larger SALT2 stretch $x_1$ ($7.91\sigma$) and larger $r$-band secondary-maximum flux $\mathcal{F}_{r_2}$ ($6.25\sigma$), while differences in SALT2 color $c$ are weak ($0.57\sigma$). Early-excess events also favor bluer $(g-z)_{\rm local}$ ($3.41\sigma$) and lower $\log_{10} (M_*/M_\odot)_{\rm local}$ ($2.73\sigma$). Our results connect early excesses with SNe~Ia diversity, and motivate further analyses of upcoming larger samples.

==> images/bumps_deluxetable.tex <==
\begin{deluxetable*}{lrrr}
\tablecaption{Bump candidates with coordinates, redshift, and fit diagnostics.\label{tab:bumps_coords}}
\tablehead{
  \colhead{ZTF name} & \colhead{$z$} & \colhead{$N_{\rm cut}^{\rm best}$} & \colhead{$\Delta{\rm BIC}$} \\
}
\startdata
  ZTF18AAIYKOZ & 0.031 & 7 & 256 \\
  ZTF18AASDTED & 0.018 & 7 & 888 \\
  ZTF18AASLHXT & 0.055 & 7 & 40 \\
  ZTF18AAYJVVE & 0.047 & 7 & 62 \\
  ZTF18ABAUPRJ & 0.024 & 7 & 2540 \\
  ZTF18ABCFLNZ & 0.027 & 7 & 54 \\
  ZTF18ABEECWE & 0.039 & 7 & 67 \\
  ZTF18ABFHRYC & 0.032 & 7 & 476 \\
  ZTF18ABJVHEC & 0.057 & 7 & 8 \\
  ZTF18ABPAYWM & 0.044 & 7 & 83 \\
  ZTF18ABUCVBF & 0.055 & 7 & 95 \\
  ZTF18ABUHYJV & 0.047 & 7 & 97 \\
  ZTF18ABUHZFC & 0.038 & 7 & 40 \\
  ZTF18ABUQUGW & 0.031 & 7 & 172 \\
  ZTF18ACCNDXN & 0.031 & 7 & 82 \\
  ZTF19AAWMQTD & 0.056 & 7 & 91 \\
  ZTF19AAXFZAO & 0.048 & 7 & 84 \\
  ZTF19AAYFAUM & 0.024 & 7 & 792 \\
  ZTF19ABDOZNH & 0.027 & 7 & 112 \\
  ZTF19ABGLMPF & 0.035 & 7 & 12 \\
  ZTF19ABMYLXW & 0.045 & 7 & 27 \\
  ZTF19ABVANIM & 0.060 & 7 & 29 \\
  ZTF19ACCMBOE & 0.046 & 7 & 42 \\
  ZTF20AAGHLKV & 0.030 & 7 & 198 \\
  ZTF20AAHKGCZ & 0.041 & 7 & 153 \\
  ZTF20AANYXVU & 0.047 & 7 & 36 \\
  ZTF20AAOSOCT & 0.059 & 7 & 55 \\
  ZTF20AAQPXTM & 0.052 & 7 & 51 \\
  ZTF20AAWDJLP & 0.027 & 7 & 72 \\
  ZTF20AAWQYWR & 0.050 & 7 & 16 \\
  ZTF20AAZYMXI & 0.036 & 10 & 89 \\
  ZTF20ABBHYXU & 0.032 & 8 & 80 \\
  ZTF20ABELJUJ & 0.048 & 7 & 56 \\
  ZTF20ABSVTNC & 0.033 & 7 & 44 \\
  ZTF20ABSZZLP & 0.029 & 7 & 90 \\
  ZTF20ABVOWVW & 0.053 & 7 & 17 \\
  ZTF20ABWEEDO & 0.039 & 7 & 29 \\
  ZTF20ABXGWJR & 0.040 & 7 & 35 \\
  ZTF20ABYGIGY & 0.059 & 10 & 62 \\
  ZTF20ACBOVRT & 0.056 & 7 & 19 \\
  ZTF20ACJHHQX & 0.055 & 7 & 35 \\
  ZTF20ACTDDOH & 0.015 & 7 & 108 \\
\enddata
\tablecomments{Coordinates are in decimal degrees. $z$ is rounded to the nearest 0.001.}
\end{deluxetable*}
